When Contracts Meets Crypto: Exploring Developers' Struggles with Ethereum Cryptographic APIs

To empower smart contracts with the promising capabilities of cryptography, Ethereum officially introduced a set of cryptographic APIs that facilitate basic cryptographic operations within smart contracts, such as elliptic curve operations. However, since developers are not necessarily cryptography experts, requiring them to directly interact with these basic APIs has caused real-world security issues and potential usability challenges. To guide future research and solutions to these challenges, we conduct the first empirical study on Ethereum cryptographic practices. Through the analysis of 91,484,856 Ethereum transactions, 500 crypto-related contracts, and 483 StackExchange posts, we provide the first in-depth look at cryptographic tasks developers need to accomplish and identify five categories of obstacles they encounter. Furthermore, we conduct an online survey with 78 smart contract practitioners to explore their perspectives on these obstacles and elicit the underlying reasons. We find that more than half of practitioners face more challenges in cryptographic tasks compared to general business logic in smart contracts. Their feedback highlights the gap between low-level cryptographic APIs and high-level tasks they need to accomplish, emphasizing the need for improved cryptographic APIs, task-based templates, and effective assistance tools. Based on these findings, we provide practical implications for further improvements and outline future research directions.

==> 6_APIMisuse.tex <==

\section{Answer to RQ3}
\label{sec:RQ3}
In this section, we conducted a study on real-world security analysis reports and define the crypto API misuses in Ethereum smart contracts.




\subsection{Data Collection and Processing}
We collected xxxx open-source audit reports on Etherscan, coming from xx security audit companies.
Then, we employed the same keywords used in Section~\ref{sec:s3-data-collection} to check whether the audit report contains crypto-related information.   
As a result, we identified 924 Hash-related reports, 676 Signature-related reports and 16 ZKP-related reports.
To make manual analysis feasible, we randomly sampled 100 reports for both Hash-related and Signature-related reports, while including all 16 ZKP-related reports.

To investigate the categories of Ethereum crypto API misuses, two authors manual analyzed these sampled audit reports, using a hybrid card sorting approach. Specifically, we include all 5 crypto-related vulnerabilities (SWC-117, SWC-120, SWC-121, SWC-122, SWC-133) in the SWC list as pre-defined categories, while also allow to create new categories if necessary. In particular, in lines with previous studies~\cite{eip-712}~\cite{defcon}, we divided SWC-121 (Missing Protection against Signature Replay Attacks) into 3 types, \emph{i.e.}, inter-contract, cross-contract, and cross-chain signature replay to characterize different attack vectors it mentioned.
Similar to Section~\ref{sec:common-task}, two authors first analyzed 40\% reports to define all categories of misuses, and then classified the remaining 60\% reports into these defined categories.
Finally, they reached agreement on the result presented in Table~\ref{table:misuse}.


\subsection{Results}

\begin{table*}[t]

	\caption{Taxonomy of common Ethereum crypto API misuses}
	
	\begin{tabular}{llcl}
		\toprule
		\textbf{Category}                                                & \textbf{Sub-Category}      & \textbf{\makecell[c]{Related \\SWC}} & \textbf{Related CWE}                                                 \\ \midrule
		\multirow{5}{*}{\makecell[l]{Missing Protection \\against Signature\\ Replay Attacks}}         & Inter-Contract Replay      & SWC-121              & CWE-294: Authentication Bypass by Capture-replay                   \\ \cmidrule{2-4}
		\multicolumn{1}{c}{}                                             & Cross-Contract Replay      & SWC-121              & CWE-294: Authentication Bypass by Capture-replay                            \\ \cmidrule{2-4}
  		\multicolumn{1}{c}{}                                             & Cross-Chain Replay      & SWC-121              & CWE-294: Authentication Bypass by Capture-replay                            \\ \cmidrule{2-4}
		\multicolumn{1}{c}{}                                             & Front-Running Replay      & --                  &             CWE-294: Authentication Bypass by Capture-replay    \\ \midrule
		\multirow{4}{*}{\makecell*[l]{Lack of Proper \\Signature \\ Verification}}
		& Missing Cryptographic Step &      SWC-122            & CWE-325: Missing Cryptographic Step                                  \\ \cmidrule{2-4}
		
		& Signature Ambiguity        & --                 & \makecell[l]{CWE-349: Acceptance of Extraneous Untrusted Data With Trusted Data}    \\ \cmidrule{2-4}
		& Signature Malleability     & SWC-117              & CWE-345: Insufficient Verification of Data Authenticity	                                 \\ \cmidrule{1-4}
		\multirow{4}{*}{\makecell[l]{Lack of Proper\\ Zero-knowledge \\Proof Verification}}       
		& Missing Cryptographic Step & --                  & CWE-325: Missing Cryptographic Step                                   \\ \cmidrule{2-4}
		& Proof Ambiguity            & --                  & \makecell[l]{CWE-349: Acceptance of Extraneous Untrusted Data With Trusted Data}  \\ \cmidrule{2-4} 
		& Proof Malleability         & --                 &  CWE-345: Insufficient Verification of Data Authenticity       \\ \cmidrule{1-4}
		\multicolumn{2}{l}{Hash Collisions With Variable Length Arguments}         & SWC-133              & CWE-759: Use of a One-Way Hash without a Salt                     \\   \cmidrule{1-4}
		
		\multicolumn{2}{l}{Weak Sources of Randomness}                 & SWC-120              & \makecell[l]{CWE-1241: Use of Predictable Algorithm in Random Number Generator}    \\ \bottomrule
	\end{tabular}
	\label{table:misuse}
\end{table*}

\subsubsection{Crypto API Misuses}
\

As shown in Table~\ref{table:misuse}, we have discovered five categoires of Ethereum crypto API Misuses, and further divided them into 12 sub-categories based on different attack vectors.
Notably, we identified five sub-categories of misuses that have not been documented in the SWC list, indicating a common oversight of them. 
To heighten developers' awareness of these newly identified sub-categories of misuses, we describe them with detailed description, examples and possible solutions.
For the remaining seven sub-categories of misuses, we follow the same definitions with the SWC list and leave them in the online supplementary materials (TODO).


\myparagraph{Front-Running Signature Replay}
\textbf{Description: }Signatures have been widely used as access control tokens in smart contracts: anyone who possesses a valid signature can attach it in the transaction input data, thus allowing  smart contracts to perform sensitive operations such as transfer.
However, these implementations might be vulnerable to front-running attacks. 
Since Ethereum transactions require some time before they are mined, a malicious miner can intercept the attached signature from transaction pending pool, initiate a new transaction, and preemptively use the signature.
Different from other signature replays in which anyone can capture and replay on-chain public signatures, front-running signature replays require the adversary capability to access the transaction pending pool and re-order the transactions.
\textbf{Example: }An audit report~\cite{pine} pointed out this misuse in a lending platform. Anyone who captures the signatures can use them and successfully receive tokens.
\textbf{Solution: }include the signature receiver (\emph{i.e.}, the token spender) in the signed message.

\myparagraph{Signature Ambiguity}
\textbf{Description: }Signature ambiguity refers to the misuses in which the signed messages fail to precisely define the semantic of the on-chain operations.
\textbf{Example: }As shown in an audit report~\cite{thetanarena}, the semantic of a signed message might be allowing the users to buy an NFT at a specific ~\emph{price}. However, in this misuse, the ~\emph{price} is not actually tied to the signature, letting requests with the same signature but different ~\emph{price} pass the verification.
\textbf{Solution: }Include all variables determining the sensitive operations into the signed message.

\myparagraph{Missing Cryptographic Step for Proof Verification}
\textbf{Description: }Zero-knowledge proof are complex systems requiring multiple cryptographic checks. 
This misuse refers to using incomplete cryptographic checks to verify the zero-knowledge proofs. It may let invalid proofs bypass the verification.
\textbf{Example: }An audit report~\cite{aztec-consensys} pointed out a lack of elliptic curve pairing check in the implementation of a zkp protocol. It allows the adversary bypass the proof verification and raise the balance for free. 
\textbf{Solution: }Always follow the standard protocols and implement all required checks step by step.

\myparagraph{Proof Ambiguity}
\textbf{Description: }Proof ambiguity are similar to signature ambiguity.
It refers to the misuses in which the public input of the proofs fail to uniquely define the semantic of the on-chain operations.
\textbf{Example: }An example of proof ambiguity can be seen in the audit report~\cite{aztec-trailsofbits}, where a variable called \emph{validatorAddress} is not tied to the proof, so the attacker can arbitrarily set this variable.
\textbf{Solution: }Include all variables determining the sensitive operations into the public input of the proof.


\myparagraph{Proof Malleability}
\textbf{Description: }This misuse refers to missing protection against proof malleability~\cite{chase2012malleable} during the proof verification.
\textbf{Example: }
For example, previous studies~\cite{groth2017snarky}~\cite{baghery2021another}shown anyone can generate a new Groth16 proof $\pi'=(A',B',C')$ based on a valid proof $\pi=(A,B,C)$ by simple algebraic transformation, so protective solutions such as signed proof should be adopted.
Another example is proof malleability caused by wrap-around errors when operating a finite field $F_q$.
 Several famous projects including snarkjs~\cite{belles2022circom} and zokrates~\cite{eberhardt2018zokrates} have suffered proof malleability due to this misuse. Given a valid proof for public input $x$, they did not check $x$ is smaller than the scalar field size $q$ of the curve $alt\_bn128$. However, since $x+q \equiv x \mod q$, changing the public input from $x$ to $x+q$ will not change the validity of the proof, causing a new valid proof passing the verification.
\textbf{Solution: }The possible solution is: adopt protective solutions~\cite{g16malleability} when using malleable proofs, and check the range of all field elements.


It is worth noting that except these defects identified from real-world audit reports, there might also be threats that theoretically exist but lack real-world evidences.
For example, any cryptographic tasks that require multi-step check might suffer the ``missing cryptographic steps'' misuse.
However, while it is infeasible to enumerate all potential threats faced by such diverse practices, our study characterizes the most practically concerned defects in the real-world.
It can serve as a solid starting point for developing security tools and enhancing the security of this ever-evolving field.

\subsubsection{Detecting crypto-related defects}
\

Despite of the diversity of crypto API misuses, we found that most misuses cannot be detected by existing audit tools. 
Specifically, we adopt the categories of machine-auditable bugs in a recent work~\cite{zhang2023demystifying}, which is derivated from a literature review of papers published on top-tier Software Engineering, Security, and Programming Language venues from 2017 to 2022. We found that only the ``weak sources of randomness'' misuse is included in the 17 categories of machine-auditable bugs, suggesting a lack of tools to detect crypto API misuses in practice.

\vspace{0.5em}
\obs{13: } \textit{
	We identified 12 types of crypto API misuses from real-world audit reports. Only 7 of them are included in the SWC list and 1 of them can be detected by existing audit tools, highlighting the lack of knowledge and available tools to mitigate these threats.
}
\vspace{0.5em}






	






